The Power of Simple Tabulation Hashing

Randomized algorithms are often enjoyed for their simplicity, but the hash functions used to yield the desired theoretical guarantees are often neither simple nor practical. Here we show that the simplest possible tabulation hashing provides unexpectedly strong guarantees. The scheme itself dates back to Carter and Wegman (STOC'77). Keys are viewed as consisting of c characters. We initialize c tables T_1, ..., T_c mapping characters to random hash codes. A key x=(x_1, ..., x_q) is hashed to T_1[x_1] xor ... xor T_c[x_c]. While this scheme is not even 4-independent, we show that it provides many of the guarantees that are normally obtained via higher independence, e.g., Chernoff-type concentration, min-wise hashing for estimating set intersection, and cuckoo hashing.

==> bloomier-save.tex <==
\begin{comment}

\section{Hard Instance in Cuckoo Hashing}

The hard instance is the 3-dimensional cube $[n^{1/3}]^3$. Here is a
sufficient condition for cuckoo hashing to fail:
\begin{itemize}
\item there exist $a,b,c \in [n^{1/3}]^2$ with $h_1(a)=h_1(b)=h_1(c)$;
\item there exist $x,y \in [n^{1/3}]$ with $h_2(x) = h_2(y)$.
\end{itemize}

If both happen, then the elements $ax, ay, bx, by, cx, cy$ cannot be
hashed. Indeed, on the left side $h_1(a)=h_1(b)=h_1(c)$ so they only
occupy 2 positions. On the right side, $h_2(x)=h_2(y)$ so they only
occupy 3 positions. In total they occupy $5<6$ positions.

The probability of 1.~is roughly $(n^{2/3})^3 / n^2 = \Omega(1)$. This
is because tabulation (on two characters) is 3-independent.

The probability of 2.~is roughly $(n^{1/3})^2 / n = 1 / n^{1/3}$.

So overall tabulation-based cuckoo hashing fails with probability
$\Omega(1 / \sqrt[3]{n})$.

%To get the stash version, consider the set $A\times B\times C$ where
%$|C| = n^\eps$. If we have a 3-way collision in $A$, and a 2-way
%collision in $B$, we will have $|C|$ nasty configurations. This
%happens with probability roughly $\big( |A|^3 / n^2 \big) \big( |B|^2
%/ n \big)$. Setting $|A| = n^{2/3}$ and $|B| = n^{1/3 - \eps}$, the
%probability is $n^{-1/3 + 2\eps}$.

%It follows easily that Simple++ doesn't fix the problem, and you still
%have roughly $n^{-1/3 + O(1/q)}$ failure probability. In fact, you
%need to rehash on $\Omega(q)$ characters for the counterexample to
%stop working (that's what Simple-Simple does!).

\subsection{Bloomier Filters}

We want a static dictionary containing $n$ data items, each with $k$
bits of associated information. If we only care about retrieving data
for elements in the set (and never run membership queries), the
optimal space is $\Theta(nk)$ bits. This can be achieved by the power
of two choices: with constant probability, the graph induced by the
two hash functions have no cycle. So we can solve a system of equations
and set the values in the two arrays, making the data associated to
$x$ be $A[h_1(x)] \oplus B[h_2(x)]$.

The following lemma suggests that, for Bloomier filters with simple
tabulation, one shouldn't try to reach a state with zero
cycles. Instead, we will later upper bound the expected number of
cycles to $f(c)$. Thus, you should just use a stash of constant size
to break the cycles.

\begin{lemma}
The expected number of cycles is $2^{\Omega(c)}$.
\end{lemma}

\begin{proof}
Our set is the $c$-dimensional cube $[n^{1/c}]^c$. Let $a,b$ be
half-keys on some $c/2$ positions, at maximal Hamming distance
$c/2$. Let $c,d$ be half-keys on the other $c/2$ positions at maximal
Hamming distance. We will look for length-4 cycles of the form $ab
\leadsto ac \leadsto db \leadsto dc$. These form a cycle iff $h_1(a) =
h_1(d)$ and $h_2(b) = h_2(c)$, which happens with probability
$1/(2n)^2$.  For a fixed set of character positions, there are
$\sqrt{n}$ choices for $a$ and $(n^{1/c} - 1)^{c/2} = (1-o(1)) \cdot
\sqrt{n}$ choices for $b$. Similarly for $(c,d)$. Thus, for a fixed
partitioning of the characters into two sets, we expect $1/4 - o(1)$
cycles of this form. There are $\binom{c}{c/2}$ partitioning. We know
we are not double-counting any cycle, since $(a,b)$ and $(c,d)$ are at
maximal Hamming distances. So we expect $2^{\Omega(c)}$ cycles of this
special form.
\end{proof}

%I think Simple++ improves this behavior significantly, and you have no
%cycle with constant probability.

\begin{theorem}
Bloomier filters with a stash of $f(c)$ can be constructed with
$\Omega(1)$ probability.
\end{theorem}

\begin{proof}
We have shwon that if tables have load $2^{-\alpha}$, the probability
that there exists a chain of length $k$ is $\le \max \{
O(\frac{1}{n}), 2^{k\alpha - O(c\lg k)} \}$.

Using the normal load of $\frac{1}{2}$, we deduce that, with
probability $1-\eps$, there is no bad chain of length $\gg c\lg
c$. Now it remains to deal with bad chains of length $O(c\lg c)$.

We claim that, with probability $1-\eps$, the maximum number of
disjoint bad chains is at most some $f(q)$. Then, the following
algorithm can construct a Bloomier filter with stash $f(q)$: find a
chain; move it all to stash; repeat. If the stash fills, rehash.

Assume for contradiction that, with probability $\eps$, there exist
$f(c)$ disjoint bad chains. Then, with probability $\ge 1-2\eps$,
there exist at least $f(c)$ disjoint bad chains of length $O(c\lg c)$.
We subsample the set of keys randomly, keeping a fraction $2^{-c}$ of
them. Fix the hash functions to some arbitrary values. After
subsampling, each chain of length $k$ survives with probability
$2^{-ck}$, so any chain survives with probability $2^{-O(c^2 \lg c)} =
c^{-O(c^2)}$. Since the chains are disjoint, so these probabilities
are independent. Thus, if there are $C \ge c^{O(c^2)}$ chains, one
survives with probability $1-\eps$. Averaging over the hash functions
and the subsampling, a bad chain remains with probability at least
$1-3\eps$. So we can fix the subsampling and maintain this
probability. That is, there exists a fixed set of size $n/2^c$ that
has a bad chain with probability $1-3\eps$. But this contradicts the
encoding bound, which shows that no cycles of any length $k\ge 2$
exists with probability more than $\eps$ when the density is so small.
\end{proof}

\end{comment}

